On the stochastic Magnus expansion and its application to SPDEs

We derive the stochastic version of the Magnus expansion for linear systems of stochastic differential equations (SDEs). The main novelty with respect to the related literature is that we consider SDEs in the It\^o sense, with progressively measurable coefficients, for which an explicit It\^o-Stratonovich conversion is not available. We prove convergence of the Magnus expansion up to a stopping time {\tau} and provide a novel asymptotic estimate of the cumulative distribution function of t. As an application, we propose a new method for the numerical solution of stochastic partial differential equations (SPDEs) based on spatial discretization and application of the stochastic Magnus expansion. A notable feature of the method is that it is fully parallelizable. We also present numerical tests in order to asses the accuracy of the numerical schemes.

==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/ctimes.tex <==
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Method}} &\text{\textbf{Log}} &\text{\textbf{Matrix Exp}} &\text{\textbf{Total}}\\
\toprule\\
\text{euler} & 0 & 0 & 5.53773 \\
\text{m1} & 0.0096901 & 0.430865 & 0.440555 \\
\text{m2} & 0.0176436 & 0.501851 & 0.519495 \\
\text{m3} & 0.0310248 & 0.441733 & 0.472758 \\
\end{tabular}


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/error_plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/error_plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/error_plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/error_plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/error_plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/error_plot_5.eps}
\end{landscape}


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/errors.tex <==
\begin{compactenum}
\item Errors for $X(1,1,:,:)$:
\begin{compactenum}
\item Reference method: euler\\
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule
(abs error) L2 &$0.126904$ &$0.0110381$ &$0.00439121$ \\
(rel error) min &$0$ &$0$ &$0$ \\
(rel error) max &$0.205907$ &$0.01839$ &$0.00683066$ \\
(rel error) mean &$0.0625635$ &$0.00421852$ &$0.00196504$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(1,2,:,:)$:
\begin{compactenum}
\item Reference method: euler\\
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule
(abs error) L2 &$0.243383$ &$0.0280747$ &$0.00685871$ \\
(rel error) min &$0.0264348$ &$0.00486868$ &$0.00486652$ \\
(rel error) max &$0.859631$ &$0.102819$ &$0.0243329$ \\
(rel error) mean &$0.352291$ &$0.0304985$ &$0.00874374$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(2,1,:,:)$:
\begin{compactenum}
\item Reference method: euler\\
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule
(abs error) L2 &$0.138459$ &$0.0100774$ &$0.00249039$ \\
(rel error) min &$0.0202317$ &$0.00294586$ &$0.00301064$ \\
(rel error) max &$0.472898$ &$0.0320305$ &$0.00657077$ \\
(rel error) mean &$0.214602$ &$0.0116499$ &$0.00403897$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(2,2,:,:)$:
\begin{compactenum}
\item Reference method: euler\\
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule
(abs error) L2 &$0.284006$ &$0.00707772$ &$0.00587619$ \\
(rel error) min &$0$ &$0$ &$0$ \\
(rel error) max &$0.283497$ &$0.00574102$ &$0.00473894$ \\
(rel error) mean &$0.0981221$ &$0.00214937$ &$0.00198676$ \\
\end{tabular}
\end{compactenum}
\item Total Errors:
\begin{compactenum}
\item Reference method: euler\\
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Method}} & \text{$\mathbb{E}[Err_{0.75}]$}\\
\toprule
m1 &$14.8\,\%$ \\
m2 &$0.951\,\%$ \\
m3 &$0.371\,\%$ \\
\end{tabular}
\end{compactenum}
\end{compactenum}


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/input.tex <==
\section{Magnus expansion for $A$, $B$ constant and deterministic}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/model.tex}
\subsection{Parameters}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/param.tex}
\subsection{Computational Times}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/ctimes.tex}
\subsection{Errors}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/errors.tex}
\subsection{Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plots.tex}
\subsection{Error Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/error_plots.tex}


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/model.tex <==
We will concern ourselves with the following SDE:
\begin{align*}
	 dX_t = B X_t dt + A X_t dW_t
\end{align*}
with\begin{align*}
A=
\left[\begin{array}[c]{*{2}{c}}
0.335302 &-0.645492 \\
-0.264419 &0.634641 \\
\end{array}\right]
\end{align*}
 and 
\begin{align*}
B=
\left[\begin{array}[c]{*{2}{c}}
-0.0572262 &0.0493763 \\
-0.665366 &0.742744 \\
\end{array}\right]
\end{align*}
The spectral norm of $A$ is $1$.
and the spectral norm of $B$ is $1$.


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/param.tex <==
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Parameter}} & \text{\textbf{value}}\\
\toprule\\
$t_0$ & $0$\\
$T$ & $0.75$\\
\verb+N_fine+ & $7501$\\
$N$ & $76$\\
\verb+M_fine+ & $1000$\\
$M$ & $1000$\\
$d$ & $2$\\
\end{tabular}


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_5.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_6.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_7.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_8.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_9.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_10.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_11.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/AB_const/Pdf/temp/plot_12.eps}
\end{landscape}


==> Figures/AB_const_T0.75_d2_N76_Neuler7501_M1000/total_err_tab.tex <==
\begin{tabular}{@{}*{1}{c}@{}}
\text{\ $\mathbb{E}[Err_{0.75}]$}\\
\toprule
\ $14.8\,\%$ \\
\ $0.951\,\%$ \\
\ $0.371\,\%$ \\
\end{tabular}%


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/ctimes.tex <==
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Method}} &\text{\textbf{Log}} &\text{\textbf{Matrix Exp}} &\text{\textbf{Total}}\\
\toprule\\
\text{exact} & 0 & 0 & 0.546463 \\
\text{euler} & 0 & 0 & 3.43363 \\
\text{m1} & 0.0213848 & 0.466337 & 0.487722 \\
\text{m2} & 0.0162298 & 0.384079 & 0.400309 \\
\text{m3} & 0.025615 & 0.392656 & 0.418271 \\
\end{tabular}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/error_plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/error_plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/error_plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/error_plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/error_plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/error_plot_5.eps}
\end{landscape}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/errors.tex <==
\begin{compactenum}
\item Errors for $X(1,1,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.0462325$ &$4.86982$ &$0$ &$0$ \\
(rel error) min &$0$ &$0$ &$0$ &$0$ \\
(rel error) max &$0.0200719$ &$3.48169$ &$0$ &$0$ \\
(rel error) mean &$0.0100004$ &$1.00831$ &$0$ &$0$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(1,2,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.0074795$ &$0.679181$ &$0.143648$ &$0.102496$ \\
(rel error) min &$0.0031229$ &$0.219262$ &$0.0262233$ &$0.0462576$ \\
(rel error) max &$0.0412319$ &$1.52529$ &$0.36606$ &$0.137071$ \\
(rel error) mean &$0.0171872$ &$0.579768$ &$0.144016$ &$0.056648$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(2,2,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.00459871$ &$0.288029$ &$0$ &$0$ \\
(rel error) min &$0$ &$0$ &$0$ &$0$ \\
(rel error) max &$0.00490722$ &$0.454991$ &$0$ &$0$ \\
(rel error) mean &$0.00247645$ &$0.16226$ &$0$ &$0$ \\
\end{tabular}
\end{compactenum}
\item Total Errors:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Method}} & \text{$\mathbb{E}[Err_{0.75}]$}\\
\toprule
euler &$0.893\,\%$ \\
m1 &$69.8\,\%$ \\
m2 &$1.71\,\%$ \\
m3 &$0.783\,\%$ \\
\end{tabular}
\end{compactenum}
\end{compactenum}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/input.tex <==
\section{Magnus expansion for $A_t\in \mathbb{R}^{2,2}$, $B=0$ deterministic}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/model.tex}
\subsection{Parameters}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/param.tex}
\subsection{Computational Times}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/ctimes.tex}
\subsection{Errors}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/errors.tex}
\subsection{Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plots.tex}
\subsection{Error Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/error_plots.tex}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/model.tex <==
We will concern ourselves with the following SDE:
\begin{align*}
	 dX_t = A_t X_t dW_t
\end{align*}
with
\begin{align*}
A_t=
\left[
\begin{array}[c]{cc}
f^{11}(t) & f^{12}(t)\\
0 & f^{22}(t)
\end{array}
\right]
\end{align*}
Here we chose:\begin{align*}
f^{11}(t)\equiv 2,
f^{12}(t)= t,
f^{22}(t)\equiv -1,
\end{align*}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/param.tex <==
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Parameter}} & \text{\textbf{value}}\\
\toprule\\
$t_0$ & $0$\\
$T$ & $0.75$\\
\verb+N_fine+ & $7501$\\
$N$ & $76$\\
\verb+M_fine+ & $1000$\\
$M$ & $1000$\\
$d$ & $2$\\
\end{tabular}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_5.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_6.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_7.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_8.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_9.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_10.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_11.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_12.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_13.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_14.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_fix/Pdf/temp/plot_15.eps}
\end{landscape}


==> Figures/B0_fix_T0.75_d2_N76_Neuler7501_M1000/total_err_tab.tex <==
\begin{tabular}{@{}*{1}{c}@{}}
\text{\ $\mathbb{E}[Err_{0.75}]$}\\
\toprule
\ $0.893\,\%$ \\
\ $69.8\,\%$ \\
\ $1.71\,\%$ \\
\ $0.783\,\%$ \\
\end{tabular}%


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/ctimes.tex <==
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Method}} &\text{\textbf{Log}} &\text{\textbf{Matrix Exp}} &\text{\textbf{Total}}\\
\toprule\\
\text{exact} & 0 & 0 & 0.623717 \\
\text{euler} & 0 & 0 & 3.59479 \\
\text{m1} & 0.0123928 & 0.389857 & 0.40225 \\
\text{m2} & 0.0537861 & 0.402788 & 0.456574 \\
\text{m3} & 0.18592 & 0.38648 & 0.5724 \\
\end{tabular}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/error_plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_5.eps}
\end{landscape}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/errors.tex <==
\begin{compactenum}
\item Errors for $X(1,1,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.00472414$ &$0.267847$ &$0.000992092$ &$0.000992092$ \\
(rel error) min &$0$ &$0$ &$0$ &$0$ \\
(rel error) max &$0.00459909$ &$0.425385$ &$0.000717248$ &$0.000717248$ \\
(rel error) mean &$0.00241371$ &$0.156724$ &$0.000243409$ &$0.000243409$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(1,2,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.00130588$ &$0.0389292$ &$0.00919457$ &$0.00365924$ \\
(rel error) min &$0.000115462$ &$0.138253$ &$0.0208161$ &$0.0206787$ \\
(rel error) max &$0.0117534$ &$0.366003$ &$0.0951578$ &$0.0816274$ \\
(rel error) mean &$0.00455276$ &$0.147693$ &$0.0310929$ &$0.0149525$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(2,2,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.000974223$ &$0.0504697$ &$0.000294412$ &$0.000294412$ \\
(rel error) min &$0$ &$0$ &$0$ &$0$ \\
(rel error) max &$0.00115177$ &$0.0926624$ &$0.000333989$ &$0.000333989$ \\
(rel error) mean &$0.000603673$ &$0.0356632$ &$0.000114646$ &$0.000114646$ \\
\end{tabular}
\end{compactenum}
\item Total Errors:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Method}} & \text{$\mathbb{E}[Err_{0.75}]$}\\
\toprule
euler &$0.23\,\%$ \\
m1 &$13.6\,\%$ \\
m2 &$0.267\,\%$ \\
m3 &$0.131\,\%$ \\
\end{tabular}
\end{compactenum}
\end{compactenum}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/input.tex <==
\section{Magnus expansion for $A\in \mathbb{R}^{2,2}$, $B=0$ deterministic}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/model.tex}
\subsection{Parameters}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/param.tex}
\subsection{Computational Times}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/ctimes.tex}
\subsection{Errors}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/errors.tex}
\subsection{Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plots.tex}
\subsection{Error Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plots.tex}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/model.tex <==
We will concern ourselves with the following SDE:
\begin{align*}
	 dX_t = A_t X_t dW_t
\end{align*}
with
\begin{align*}
A_t=
\left[
\begin{array}[c]{cc}
f^{11}(t) & f^{12}(t)\\
0 & f^{22}(t)
\end{array}
\right]
\end{align*}
Here we chose:
\begin{align*}
A_t=\frac{\tilde{A}_t}{\sigma(\tilde{A}_t)},\end{align*}
where $\sigma(A_t)$ is the spectral radius and 
\begin{align*}
\tilde{A}_t=
\left[
\begin{array}[c]{cc}
2 & t\\
0 & -1
\end{array}
\right]
\end{align*}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/param.tex <==
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Parameter}} & \text{\textbf{value}}\\
\toprule\\
$t_0$ & $0$\\
$T$ & $0.75$\\
\verb+N_fine+ & $7501$\\
$N$ & $76$\\
\verb+M_fine+ & $1000$\\
$M$ & $1000$\\
$d$ & $2$\\
\end{tabular}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_5.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_6.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_7.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_8.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_9.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_10.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_11.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_12.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_13.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_14.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_15.eps}
\end{landscape}


==> Figures/B0_var_T0.75_d2_N76_Neuler7501_M1000/total_err_tab.tex <==
\begin{tabular}{@{}*{1}{c}@{}}
\text{\ $\mathbb{E}[Err_{0.75}]$}\\
\toprule
\ $0.23\,\%$ \\
\ $13.6\,\%$ \\
\ $0.267\,\%$ \\
\ $0.131\,\%$ \\
\end{tabular}%


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/ctimes.tex <==
\begin{tabular}{@{}*{4}{c}@{}}
\text{\textbf{Method}} &\text{\textbf{Log}} &\text{\textbf{Matrix Exp}} &\text{\textbf{Total}}\\
\toprule\\
\text{exact} & 0 & 0 & 8.19245 \\
\text{euler} & 0 & 0 & 42.8796 \\
\text{m1} & 0.0358899 & 5.01931 & 5.0552 \\
\text{m2} & 0.0918883 & 4.92811 & 5.01999 \\
\text{m3} & 0.249613 & 4.99174 & 5.24135 \\
\end{tabular}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/error_plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plot_5.eps}
\end{landscape}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/errors.tex <==
\begin{compactenum}
\item Errors for $X(1,1,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.0628271$ &$18.5607$ &$0.0293314$ &$0.0293314$ \\
(rel error) min &$0$ &$0$ &$0$ &$0$ \\
(rel error) max &$0.00649982$ &$2.75525$ &$0.00252757$ &$0.00252757$ \\
(rel error) mean &$0.0603359$ &$18.7902$ &$0.0206468$ &$0.0206468$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(1,2,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.0698386$ &$15.3511$ &$4.92363$ &$1.48978$ \\
(rel error) min &$0.00307985$ &$0.215211$ &$0.00658027$ &$0.0179254$ \\
(rel error) max &$0.0189742$ &$1.70873$ &$0.618511$ &$0.27756$ \\
(rel error) mean &$0.150542$ &$11.6923$ &$3.96709$ &$1.39095$ \\
\end{tabular}
\end{compactenum}
\item Errors for $X(2,2,:,:)$:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{5}{c}@{}}
\text{\textbf{Error}} &\text{\textbf{euler}} &\text{\textbf{m1}} &\text{\textbf{m2}} &\text{\textbf{m3}} \\
\toprule\\
(abs error) L2 &$0.00768587$ &$1.24738$ &$0.00426152$ &$0.00426152$ \\
(rel error) min &$0$ &$0$ &$0$ &$0$ \\
(rel error) max &$0.0016174$ &$0.3921$ &$0.00065566$ &$0.00065566$ \\
(rel error) mean &$0.0151104$ &$2.91449$ &$0.00588822$ &$0.00588822$ \\
\end{tabular}
\end{compactenum}
\item Total Errors:
\begin{compactenum}
\item Reference method: exact\\
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Method}} & \text{$\mathbb{E}[Err_{10}]$}\\
\toprule
euler &$0.67\,\%$ \\
m1 &$90.5\,\%$ \\
m2 &$15.3\,\%$ \\
m3 &$5.18\,\%$ \\
\end{tabular}
\end{compactenum}
\end{compactenum}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/input.tex <==
\section{Magnus expansion for $A\in \mathbb{R}^{2,2}$, $B=0$ deterministic}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/model.tex}
\subsection{Parameters}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/param.tex}
\subsection{Computational Times}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/ctimes.tex}
\subsection{Errors}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/errors.tex}
\subsection{Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plots.tex}
\subsection{Error Plots}
	\input{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/error_plots.tex}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/model.tex <==
We will concern ourselves with the following SDE:
\begin{align*}
	 dX_t = A_t X_t dW_t
\end{align*}
with
\begin{align*}
A_t=
\left[
\begin{array}[c]{cc}
f^{11}(t) & f^{12}(t)\\
0 & f^{22}(t)
\end{array}
\right]
\end{align*}
Here we chose:
\begin{align*}
A_t=\frac{\tilde{A}_t}{\sigma(\tilde{A}_t)},\end{align*}
where $\sigma(A_t)$ is the spectral radius and 
\begin{align*}
\tilde{A}_t=
\left[
\begin{array}[c]{cc}
2 & t\\
0 & -1
\end{array}
\right]
\end{align*}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/param.tex <==
\begin{tabular}{@{}*{2}{c}@{}}
\text{\textbf{Parameter}} & \text{\textbf{value}}\\
\toprule\\
$t_0$ & $0$\\
$T$ & $10$\\
\verb+N_fine+ & $100001$\\
$N$ & $1001$\\
\verb+M_fine+ & $1000$\\
$M$ & $1000$\\
$d$ & $2$\\
\end{tabular}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/plots.tex <==
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_1.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_2.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_3.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_4.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_5.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_6.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_7.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_8.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_9.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_10.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_11.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_12.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_13.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_14.eps}
\end{landscape}
\begin{landscape}
\includegraphics[width=.95\columnwidth]{C:/Users/kevin/Documents/MATLAB/PhD/Magnus/Final/Correction/B0_var/Pdf/temp/plot_15.eps}
\end{landscape}


==> Figures/B0_var_T10_d2_N1001_Neuler100001_M1000/total_err_tab.tex <==
\begin{tabular}{@{}*{1}{c}@{}}
\text{\ $\mathbb{E}[Err_{10}]$}\\
\toprule
\ $0.67\,\%$ \\
\ $90.5\,\%$ \\
\ $15.3\,\%$ \\
\ $5.18\,\%$ \\
\end{tabular}%

